Efficient Pose and Cell Segmentation using Column Generation

We study the problems of multi-person pose segmentation in natural images and instance segmentation in biological images with crowded cells. We formulate these distinct tasks as integer programs where variables correspond to poses/cells. To optimize, we propose a generic relaxation scheme for solving these combinatorial problems using a column generation formulation where the program for generating a column is solved via exact optimization of very small scale integer programs. This results in efficient exploration of the spaces of poses and cells.

==> app_backup.tex <==
\section{Supplementary}
\subsection{input for our framework}

Input to our framework:

given part detection (angle, knee, hip,  wrist, elbow shoulder) neck , head

deep net (`deep cut') (input is an image; for a series of interest points we get their distribution over the  14 objects)

interest points (deep cut paper)

features with each interest point , i.e., detection

\begin{itemize}
\item input image
\item interest points
\item associate each interest point with probability distribution over labels
\item associate each pair of interest points with a probability of being part of the same object, conditioned on the two labels of those interest points
\item construct an MRF on top of this
\item solve this MRF using ILP solver (pretty big and slow)
\end{itemize}

Output of our system:
N  poses, where each pose contains a set of interest points (possibly a subset of the 14 possible parts); N is not restricted and our model will search for as many as it can find

How does our system work:
we replace the ILP solver with something significantly more effective, which works as follows:


OUTLINE OF OUR SYSTEM JULIAN

PART 1:  RECIVE INPUT FROM DEEP CUT.   I describe the system as I undertand it below.  I know part 2 (the optimizer) fully.  But I did not do the preprocesing 

step 1.  run deep net from deep cut to produce as set of detections.  \alex{I guess we should refer to those detections as keypoints?}

julian reply:  i support that. keypoints is good to me. 

step 2: For each detection we associate a unary cost to take on each label for 14 semantic labels.  

step 3:  Consider every for tuple [detection1,detection2,part1,part2] we associate a cost for detection1 and detection2 to be take on part labels part1,part2 respectively {\bf AND be associated with a common pose}.  \alex{I guess that's just a pairwise potential; although I'm not yet sure how to encode the latter part, \ie, `AND be associated with a common pose'}

julian: the encoding is done dueing the genrwtion of columns.  a column is described by a total cost and a set of detectins associated wiht it (and part labels ) 

NOTE: under the deep cut system a GAINT ILP is then solved.  This essentially is a correlation clustering problem plus assigning part labels ot detections.  Sometimes it takes weeks.

PART 2:  NOW  THIS IS WHERE OUR SYSTEM DIFFERS

\alex{What's missing is the description of the graph that we run this on, \ie, what do the nodes correspond to; we need this before describing the interactions between the nodes; also missing seems to be what do the unaries correspond to? where do they go?}

juLIAN  :unary terms are present also. remember the graph we are describing here corresponds to generating columns.  the combination ofmthe columns to describe the people in the scene is done by the lp operating given the columns. hence nodes correspond tomparts and labels for the nodes are detections.  The concept here is that set packing formulation combines the columns( POSES).  when we make a column however interactions with other poses are described entirely by lagrange multipliers which alter the unsry terms.  (TRIPLETS are a different story and they indice higher order interractions between nodes but still ony in the form of altering potentials in the mrf.  

We now associate a pairwise interaction with all connections  on the standard tree model of a part.  We also associate pairwise connection between every part and every part of a subset called the FULL SET.  This includes currently 5 of the 14 parts.  Thus we have a highly connected model.  THe full set includes all center located parts on the body:  neck shoulders and hips.  

We force every detection to be associated with exactly one part.  

We now apply column generation. 

\alex{Before we describe the algorithm we should describe the problem and at this point in time I don't see the definition of the problem yet. I understand the giant ILP. Can we use the same formulation?}

Generating rows is done only at convergence of lower bound.  

Generating columns is done by solving ILPs. 
step 1:  
We solve one ILP for every detection. This identifies the optimal vassal pose including any given detection

step 2: 

we solve one ILP for every  configuration of the master set.  Every valid queen pose includes at least one detection from teh master set of parts included.  Currenlty the master set includes the neck.  Thus every person has a neck is the imposed constraint. 

To generate as queen posewWe solve a markov random field.  This has one node for every part.  The node for a given part  has one state for every detection of a given part.  A queen pose describes  up to one detection for every part.  Non included parts are hence occluded in that queen pose.  

We do optimization until convergence which is fast.  

At each step we compute an upper bound.  This is done by solving an ILP.  IT is fast and we need not solve it every time.  Generally the LP is tight at termination or off my a small fraction of a percent 

The selection of vassal poses and queen poses describes a unique selection of complete poses even for fractional solutions.  This is NOT rounded or approximated and is easy to produce.  NO ILP or LP is  solved for this.  

Visualization is done on shaofei's end.  

OUR model

A complete pose is described by a queen pose and a set of vaassal poses.  A queen pose has one detection included for each non occluded part. A complete pose has one vassal pose for each non occluded detection in the queen pose.  Each vassal pose is associated with a subset of the detections of a the corresponding part of the vassal pose.   

The cost of a complete pose is the cost the following 3 terms:  
1.  Cost of all pariwise interactions between queen detections of that pose
2.  The unary cost of each detection included in the complete pose
3.  The cost of all pairwise interactions between each queen and their resepctive vassals.  

\section{Initial Formulation}

We define the set of all interest points as  $\mathcal{D}$

We use $\mathcal{P}$ to define the set of complete poses which we index by $p$.  We associate  each pose with a subset of the interest points .  We use a matrix  $X \in \{0,1\}^{|\mathcal{D}| \times |\mathcal{P}|}$ to describe complete poses.  Here $X_{dp}=1$ indicates that  interest point  $d$ is associated with pose $p$.   

We use $\bar{\gamma} \in \{0,1\}^{\mathcal{P}}$ to describe a selection of complete poses.  We associate  a cost vector with $\mathcal{P}$ here $\Theta \in \mathbb{R}^{\mathcal{P}}$ with $\gamma$.  We now frame selecting a set of low cost poses as set packing.  

\begin{align}
\label{intorigposilp}
\min_{\bar{gamma} \in \{ 0,1\}^{|\mathcal{P}|} }\Theta^t \bar{\gamma} \\
\nonumber X\gamma \leq 1
\end{align}

\subsection{Defining $\Theta$}

We  associate  a pose with portions denoted queen and  vassal.  For a given pose a  part that is assocaited with a interest point is associated with exactly one queen for that part.  No queen exists for that pose if the corresponding part is occluded. Similarly for each part in which there is at least two interest points associated with a given  pose  ther is a vassal pose.  

We use $X^{0Q}$ to define the queen pose of a given  complete pose.  We use  $X^{0Q}_{dp}=1$ to indicate that interest-point $d$ takes is a queen in complete pose $p$.  

The cost of a given pose  is descrbed  as the pairwise interaction between queens plus the  pairwise interactions betwen  vassals and queens of the same part within a pose.  We use $R_{d}$ to denot the part assocaited with a given interest point.  Notice that every interest point can be associated with exactly one part and this is produced not by optimiation but by the model.   (earlier versions of our model did not include this constraint but it allows for mathematical power)

We now write teh cost of a pose.

\begin{align}
\Theta_p=\sum_{d}\theta_dX_{dp}+\\
\nonumber +\sum_{d_1,d_2}\theta_{d_1,d_2}[X^{0q}_{d_1p}==X^{0q}_{d_1p}]\quad \mbox{queen to queen}\\
\nonumber +\sum_{d_1,d_2}\theta_{d_1,d_2}X_{d_1p}X_{d_2,p}[R_{d_1}=R_{d_2}] \mbox{queen/vasssal and vassal/vassal }
\end{align}
\section{Stronger Math formulation}

\subsection{Problem with the above formulation}

Our intial owrk used the formulation in Eq \ref{intorigposilp}.  However we found that this was problematic in contexts where vassal poses existed.  THus the model worked fine when each pose had not more than one interest point assoicated with a given part.  That model however did not handle non max suprression so we had to drop it.  Optimization was based on column generation adn too many columns had to be produced.  Instead we  decided to implicitly encode many  complete poses by instead describing a set of queen poses and vassal poses.  This allowed for the use of very few columns to describe very many columns.  

Instead of encoding a number of complete poses we encode a set of queen and vassal poses which can be combined to form complete poses.  
\subsection{New formulation}

We define the seq of queen/vassal poses as $\mathcal{Q}$ and $\mathcal{V}$ respectively which we index with $p$.  We describe the  queen poses using a matrix  $X^{Q} \in \mathcal{0,1}^{|\mathcal{D}| \times ||mathcal{Q} }$ which we index with $d,p$.  We use $X^Q_{dp}=1$ to indicate that  interest-point $d$ is included queen pose $p$.  

We use  $X^{V1}_{dp}=1$ to indicate that  interst-point  $d$ is  include $d$ in vassal pose $p$ and is not the queen.  We use $X^{V2}_{dp}=1$ to indicate  that  detection $d$ is the queen in vassal pose  $p$.  

We define a selection of terms  using indicator vectors $\bar{\gamma}^Q\in \{ 0,1 \}^{|\mathcal{Q}|}$ , $\bar{\gamma}^V\in \{ 0,1 \}^{|\mathcal{V}|}$ 

We note that $\bar{\gamma}^Q_p=1$ 

We seek to select a  set of low cost queen and vassal poses under the following constraints.  

1.  For any given interest point the number of selected queen poses plus the number of times it is in a vassal pose as a non queen is no more than one.  Formally this is as follows  
\begin{align}
X^Q\bar{\gamma}^Q+X^{1V}\bar{\gamma}^V \leq 1 
\end{align}

2.  For  any  given interst point  the number of selected vassal poses in which it is either a vassal or a queen is no more than one.  Formally :
\begin{align}
(X^{1V}+X^{2V})\bar{\gamma}^V \leq 1
\end{align}

3.  For any interst point  the number of  selected vassals in which  that interest point is a queen  is bounded from above by the number of queen poses inclduing that interest point.  Formally:  
\begin{align}
X^{2V}\gamma^V \leq X^{Q} \bar{\gamma}^qQ
\end{align}

Using these three constraints we write optmization 

\begin{align}
\label{integerBetterObj}
Eq \ref{intorigposilp} = \min_{\substack{\bar{\gamma}^Q  \in \{ 0,1\}^{\mathcal{Q}} \\ \bar{\gamma}^C  \in \{ 0,1\}^{\mathcal{V}}}} \Theta^{tQ} \gamma^Q+\Theta^{tV}\bar{\gamma}^V  \\
\nonumber X^Q\bar{\gamma}^Q+X^{1V}\bar{\gamma}^V \leq 1 \\
\nonumber (X^{1V}+X^{2V})\bar{\gamma}^V \leq 1 \\
\nonumber X^{2V}\gamma^V \leq X^{Q} \bar{\gamma}^qQ
\end{align}

\subsection{The LP relaxation}

Observe that   Eq \ref{integerBetterObj} is  equivelent to Eq \ref{intorigposilp} which itself is equivelent to max weight set packing  problem which is NP hard.  Thus we attack optmiztaion using the well studied tools of LP relaxations.  

We provide a convex relaxation of Eq \ref{integerBetterObj} below.  

\begin{align}
\min_{\gamma \geq 0} \Theta^{tq} \gamma^q+\Theta^{tv}\gamma^v  \\
\nonumber X^q\gamma^q+X^{1v}\gamma^v \leq 1 \\
\nonumber (X^{1v}+X^{2v})\gamma^v \leq 1 \\
\nonumber X^{2v}\gamma^v \leq X^{q} \gamma^q 
\end{align}

This LP relaxation only contains constraints for collections of poses
that share a common detection.  From the view point of maximum-weight
set packing, this includes some cliques of conflicting sets but misses many
others.

As a concrete example, 
consider four poses $\mathcal{P}=\{p_1,p_2,p_3,p_4\}$ over
three interest points  $\mathcal{D}=\{ d_1,d_2,d_3\}$ where the first three poses
each contain two of the three interest-points $\{d_1,d_2\},\{d_1,d_3\},\{d_2,d_3\}$, and
the fourth pose contains all three $\{d_1,d_2,d_3\}$.  Suppose the pose costs
are given by $\Theta_{p_1}=\Theta_{p_2}=\Theta_{p_3}=-4$ and $\Theta_{p_4}=-5$.
The optimal integer solution sets $\pmb{\gamma}_{p_4}=1$, and has a cost of
$-5$.  However a lower cost fractional solution sets
$\pmb{\gamma}_{p_1}=\pmb{\gamma}_{p_2}=\pmb{\gamma}_{p_3}=0.5$;
$\pmb{\gamma}_{p_4}=0$ which has cost $-6$.  Hence the LP relaxation is loose
in this case.

A tighter bound can be motivated by the following observation.  For any set of
three unique interest points the number of poses that include two or more
members can be no larger than one. 

We now apply our tighter bound to pose segemtation.  We denote the set of groups of three unique superpixels  (which we refer to as triplets) as
$\mathcal{C}$ and index it with $c$.  Using  $C \in \{0,1\}^{|\mathcal{C}|\times|\mathcal{P}|}$ we define a tighter space for $\gamma^Q,\gamma^V$.
\begin{align}
 C^Q \pmb{\gamma}^Q \leq 1 \}  \\
\nonumber C_{cp}=[\sum_{d \in c}X^Q_{dp}\geq 2] \quad \forall c \in \mathcal{C}, p \in \mathcal{P}\\
 C^V \pmb{\gamma}^Q \leq 1 \}  \\
\nonumber C_{cp}=[\sum_{d \in c}X^{V2}_{dp}\geq 2] \quad \forall c \in \mathcal{C}, p \in \mathcal{P}
\end{align}


\subsection{Adding in triplets}
We now write optimizatio nincluding the triplet constraints 

\begin{align}
\min_{\gamma \geq 0, \beta \geq 0} \Theta^{tq} \gamma^q+\Theta^{tv}\gamma^v  \\
\nonumber X^q\gamma^q+X^{1v}\gamma^v \leq 1 \\
\nonumber (X^{1v}+X^{2v})\gamma^v \leq 1 \\
\nonumber X^{2v}\gamma^v \leq X^{q} \gamma^q \\
\nonumber C^v\gamma^v \leq 1\\
\nonumber C^q\gamma^q \leq 1
\end{align}

\subsection{Adding in Bounds}
This section will be tough to communicate.  

\subsection{Expanded Space Column Generation}
\label{expandspace}

Since the $\mathcal{P}$ contains a massive number of member, Eq.
\ref{lpObj} is intractable. Instead we consider an
approximation using a set $\hat {\mathcal{P}}$ which is a subset of $\mathcal{P}$. 

We introduce a slack vector $\beta \geq 0$ inspired by \cite{HPlanarCC} that tracks the presence of any
``over-included'' members of $\mathcal{D}$ and prevents them from contributing to the objective when their inclusion improves the objective.  Let $\Phi_d$ be an upper bound on the increase in $\Theta_p$ for every $p$ using  $d$ if  $d$ was removed (creating an identical column except that $d$ is removd).  Formally for the case of pose it is as follows.  

NOTE:  
In practice we found it useful to enforce taht every queen pose has a t least one member of a set of master parts as a detection. We used one master part m notably the neck. 

\begin{align}
\min_{\gamma \geq 0, \beta \geq 0} \Theta^{tq} \gamma^q+\Theta^{tv}\gamma^v +\Phi^1\beta^1+\Phi^{2t}\beta^2 \\ 
\nonumber +\Phi^{3t}\beta^{3}+\Phi^{4}\beta^{4}+\Phi^{5}\beta^{5} \\
\nonumber X^Q\gamma^q+X^{1V}\gamma^v-\beta^1 \leq 1 \\
\nonumber (X^{1V}+X^{2V})\gamma^v-\beta^2 \leq 1 \\
\nonumber X^{2v}\gamma^V-\beta^{3}\leq X^{Q} \gamma^q \\
\nonumber C^v\gamma^V -\beta^{4}\leq 1\\
\nonumber C^q\gamma^Q -\beta^{5}\leq 1
\end{align}

\begin{align}
\max_{\substack{\lambda \geq 0 \\ \Phi^1 \geq \lambda^1 \\ \Phi^2 \geq \lambda^2 \\ \Phi^3 \geq \lambda^3 \\ \Phi^4 \geq \lambda^4 \\ \Phi^5 \geq \lambda^5}}-(\lambda^{1t}+\lambda^{2t}+\lambda^{4t}+\lambda^{5t})1\\
\nonumber C^{qt}\lambda^{5}+X^{qt}\lambda^{1}-X^{qt} \lambda^3 \geq 0\\
\nonumber C^q\lambda^{4}+X^{1vt}\lambda^{1}+(X^{1tv}+X^{2tv})\lambda^{2}+X^{2tv}\lambda^{3}\geq 0\\
%\nonumber \Phi^{1}\geq \lambda^{1}\\
%\nonumber \Phi^{2}\geq \lambda^{2}\\
%\nonumber \Phi^3\geq \lambda^{3}\\
%\nonumber \Phi^{4}\geq \lambda^{4}\\
%\nonumber  \Phi^{5}\geq \lambda^{5}\\
\end{align}




==> cellAppBack.tex <==


\section{Cell Instance Segmentation}

We now consdier the problem of cell segemtantion using the tools from the work on pose segmentation. The technique described in this paper is applicable to images that have crowded cell regions acquired from different modalities and cell shapes, while individual cells are mainly discernible by boundary cues. Our approach starts by generating an oversegmentation, or a set of superpixels, then it finds a clustering of the superpixels into an arbitrary number of segments such that the set of edge . Previous work~\cite{Zhang14b}...

\subsection{math formulation}
We now consider our approach based on the work of \cite{}.  Given a set of super-pixels $\mathcal{D}$, each with a
specified spatial location, our goal is to identify a collection of segmentations of individual cells.% We assume that a track trajectory
%is uniquely determined by the set of detections associated with it and that
%some detections may be false positives not associated with any track.

We denote the set of all possible cells by $\mathcal{P}$ and use $X$ to denote
the superpixel-cell incidence matrix $X \in \{ 0,1\}^{
|\mathcal{D}|\times|\mathcal{P}|}$ where $X_{dp}=1$ if and only if cell $p$
includes superpixel $d$. A solution to the cell instance segmentation problem is
denoted by the indicator vector $\pmb{\gamma} \in \{0,1\}^{|\mathcal{P}|}$ where
$\pmb{\gamma}_p=1$ indicates that cell $p$ is included in the solution and
$\pmb{\gamma}_p=0$ otherwise.  A collection of cells specified by $\pmb{\gamma}$ is a
valid solution if and only if each detection is associated with at most one active
cell.  Using $\Theta \in \mathbb{R}^{|\mathcal{P}|}$ to denote the costs
associated with cells where $\Theta_p$ describes the cost of cell $p$,
we express our instance segmentation as an integer linear program:
\begin{align}
\label{intobj}
\min_{ \pmb{\gamma} \in \bar{\pmb{\Gamma}}}\Theta^t \pmb{\gamma} 
\quad \quad \quad \text{with}
\quad \quad
\bar{\pmb{\Gamma}} = \{ {\pmb{\gamma}} \in \{ 0,1\}^{|\mathcal{P}|}: \;X {\pmb{\gamma}} \leq 1 \}
\end{align}
%Here $\bar{\pmb{\Gamma}}$ is the space of feasible (integer) solutions.
 We note that this is equivalent to finding a maximum-weight set packing  which is NP-hard~\cite{karp}.%where each
%set is a collection of detections corresponding to a track and our goal is to
%choose a collection of pairwise disjoint sets.  This problem is
%NP-hard~\cite{karp}.% and this formulation faces further difficulties as the size
%of the ILP scales exponentially in the number of detections.

\subsection{Associating Costs to Cells}
%A classic approach to scoring an individual track is to use a Markov model
%that incorporates unary scores associated with individual detections along
%with pairwise comparabilities between subsequent detections assigned to a
%track. Such an approach provides efficient inference but is limited in its
%ability to model higher-order dynamical constraints. 
% Instead,
 We consider a scoring function  mapping subsets of superpixels .  Cells are constrainted to have a maximum radius (denoted $m_R$) and a maximum  surface area (or volume) denoted $m_V$.  The inclusion of a superpixel $d$in a cell is assocaited with a cost $\theta_d$.  The inclusion of a pair of superpixels $d_1,d_2$ is assocaited with a cost $\theta_{d_1d_2}$.  The distance between a pair of superpixels$d_1,d_2$  is denoted  $L_{d_1d_2}$.The volume of a superpixel $d$ is denoted $V_d$.  A cell is associated with an offset cost $\theta_0$.  

 \begin{align}
 \Theta_p=\theta_0+\sum_{(d_1,d_2)\in \mathcal{D}}\theta_{d_1d_2}+\sum_{d\in\mathcal{D}}(\infty \min_{\hat{d}}\sum_{d \in \mathcal{D}}X_{dp}[L_{d,\hat{d}}\geq m_R])\\
 \nonumber +(\infty [m_V\leq \sum_{d\in \mathcal{D}}X_{dp}V_{d}])
 \end{align}


\subsection{LP Relaxation and Column Generation}
\label{lpclique}
We now attack optimization in Eq \ref{intobj} using the well studied tools of
LP relaxations.  We use $\pmb{\Gamma} = \{ \pmb{\gamma} \in [0,1]^{|\mathcal{P}|}: \;X \pmb{\gamma} \leq 1 \}$
to denote a convex relaxation of the constraint set $\bar{\pmb{\Gamma}}$. 
\begin{align}
\min_{ \pmb{\gamma} \in \bar{\pmb{\Gamma}}}\Theta^t \pmb{\gamma} 
\quad \geq \quad \min_{ \pmb{\gamma} \in \pmb{\Gamma}}\Theta^t \pmb{\gamma} 
\end{align}

%\label{betterLP}
This LP relaxation only contains constraints for collections of cells
that share a common detection.  From the view point of maximum-weight
set packing, this includes some cliques of conflicting sets but misses many
others.

%\subsection{Fractional solutions from mutually exclusive triplets}
As a concrete example, % we consider a case where the LP relaxation Eq
%\ref{duallp} provides a loose lower bound which is visualized in Fig
%\ref{looseExpFig}.  
consider four cells $\mathcal{P}=\{p_1,p_2,p_3,p_4\}$ over
three superpixels $\mathcal{D}=\{ d_1,d_2,d_3\}$ where the first three tracks
each contain two of the three superpixels $\{d_1,d_2\},\{d_1,d_3\},\{d_2,d_3\}$, and
the fourth cell contains all three $\{d_1,d_2,d_3\}$.  Suppose the cell costs
are given by $\Theta_{p_1}=\Theta_{p_2}=\Theta_{p_3}=-4$ and $\Theta_{p_4}=-5$.
The optimal integer solution sets $\pmb{\gamma}_{p_4}=1$, and has a cost of
$-5$.  However the optimal fractional solution sets
$\pmb{\gamma}_{p_1}=\pmb{\gamma}_{p_2}=\pmb{\gamma}_{p_3}=0.5$;
$\pmb{\gamma}_{p_4}=0$ which has cost $-6$.  Hence the LP relaxation is loose
in this case.  %Even worse, rounding the fractional solution results in a
%sub-optimal solution. 
 %
%\label{3fix}
%

A tighter bound can be motivated by the following observation.  For any set of
three unique superpixels the number of celss that include two or more
members can be no larger than one.  %Thus the following inequality holds for
%groups of three unique detections  (which we refer to as triplets)
%$d_1,d_2,d_3$.  We use $[...]$ to express the indicator function.  
%
%\begin{align}
%\label{lpcorrect3}
%\sum_{p \in \mathcal{P}}[X_{pd_1}+X_{pd_2}+X_{pd_3} \geq 2]\pmb{\gamma}_p\leq 1 
%\end{align}
%
We now apply our tighter bound to intstance segemtantion.  We denote the set of groups of three unique superpixels  (which we refer to as triplets) as
$\mathcal{C}$ and index it with $c$.  Using  $C \in \{0,1\}^{|\mathcal{C}|\times|\mathcal{P}|}$ we define a tighter space for $\pmb{\gamma}$ than $\pmb{\Gamma}$.
\begin{align}
\pmb{\Gamma}^C: \{ \pmb{\gamma} \in \mathbb{R}^{|\mathcal{P}|}: \pmb{\gamma} \geq 0,\quad X \pmb{\gamma} \leq 1, \quad C \pmb{\gamma} \leq 1 \}  \\
\nonumber C_{cp}=[\sum_{d \in c}X_{dp}\geq 2] \quad \forall c \in \mathcal{C}, p \in \mathcal{P}
\end{align}


\section{Optimization over $\pmb{\Gamma}^{C}$}
\label{tightlpopt}
We write instance segmentation as optimization in the primal and dual form below.
\begin{align}
\label{lpobjC}
\min_{\pmb{\gamma} \in \pmb{\Gamma}^C}\Theta^t\pmb{\gamma} 
=\max_{\substack{\pmb{\lambda} \geq 0\\ \pmb{\lambda}^{\mathcal{C}}\geq 0 \\ \Theta+X^t\pmb{\lambda}+ C^t\pmb{\lambda}^{\mathcal{C}} \geq 0}} -1^t\pmb{\lambda}-1^t\pmb{\lambda}^{\mathcal{C}} 
\end{align}

Given that $\mathcal{P}$ and $\mathcal{C}$ are of enormous size we use column
and row generation jointly.  The nascent subsets of $\mathcal{P},\mathcal{C}$
are denoted $\hat{\mathcal{P}}, \hat{\mathcal{C}}$ respectively.
We write column/row generation optimization given subroutines
$\mbox{COLUMN}(\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}})$,
$\mbox{ROW}(\pmb{\gamma})$ that identify a group of violated constraints in
primal and dual including the most violated in each.  We write the column/row
generation optimization  in Alg \ref{dualsolvesimplecyc}.

Rounding the final solution is not neccessary as it is generally integral.  However in cases where it is not one of many mechnsims can be used .  We used that of \cite{yarkoNips2016} however we found that practically solving  optimizing set packing over the integeral set of solutions over $\hat{\mathcal{P}}$ was practically very cheap. 

\subsection{Row Generation}
Finding the most violated row consists of the following optimization:    
%\begin{align}
$\max_{c \in \mathcal{C}}\sum_{p \in \mathcal{P}} C_{cp} \pmb{\gamma}_p$.  
%\end{align}
%
%Enumerating $\mathcal{C}$ is unnecessary and 
We generate its rows as needed by considering only  triplets over superpixels associated with fractional valued cells. %$c=\{ d_{c_1} d_{c_2} d_{c_3} \}$ such that for each of pair $d_{c_i},d_{c_j}$  there exists a fractional valued track containing both $d_{c_i}$ and $d_{c_j}$.

\subsection{Generating Columns}
\label{colbb}

We denote  the value of the slack corresponding to an arbitrary column $p$
as $V(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}},p)$ and the most
violated as $V^*(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}})$ which we
define below.   
\begin{align}
\label{Vequ}
V(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}},p)&=\Theta_p+\sum_{d \in \mathcal{D}}\pmb{\lambda}_{d} X_{dp} +\sum_{c \in \hat{\mathcal{C}}}\pmb{\lambda}^{\mathcal{C}}_c C_{cp}\\ % \\
V^*(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}})&=\min_{p \in \mathcal{P}}V(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}},p)
\label{minColOverall}
\end{align}

Optimizing  Eq \ref{minColOverall} is  a very challanging integer program.  However it can be attacked by solving $\mathcal{D}$ tiny problems exactly.  The lowest cost solution will be established to be the most violated column.  In practice all violated columns produced are added to the $\mathcal{D}$. Recall that every subset of superpixels  is associated with a centroid superpixel.  Given teh centroid of for cell the set of other superpixels that may be included is small as it is only those within the radius of the centroid.  Thus we  produce one column as follows.  

\begin{align}
V^{d*}(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}})&=\min_{\substack{p \in \mathcal{P}\\X_{dp}=1}}V(\Theta,\pmb{\lambda},\pmb{\lambda}^{\mathcal{C}},p)
\end{align}





==> cellSupplementaryInfo.tex <==
\subsection{Cell segmentation experiments}
\label{suppl:cell}

We find a detection using Hungarian matching with centroid distance, and report matches between found segments and the manually labeled ground-truth (GT) regions based on area overlap. Unmatched GT regions are false negatives (FN), unmatched segmentation regions are false positives (FP). Results are reported in terms of precision P=TP/(TP+FP), recall R=TP/(TP+FN), and F-score F=2$\times$P$\times$R/(P+R).

==> col_LP2_legacy.tex <==


\subsection{ILP Two:  Decoupling Local and Global Interactions}
%
%In this section we study an alternative ILP to  \equref{packingIlp} that is more efficient to solve in practice.  \alex{if this is more efficient to solve, why do we even discuss the first technique? seems not important then} %permits the expression of sol %can be made more efficeint by  allowing for the expression of complete poses via a dictionary of poses defining local and global interactions .  
%
In this section we discuss our column generation formulation of the integer program in Eq \ref{eq:MainProg}.  Empirically we observe that the LP relaxation of this program to be tight in practice. 

We define the set of all possible settings of global detections for a given pose as $\mathcal{Q}^1$ which we index with $q$. We describe  $\mathcal{Q}^1$ using a matrix $X^{1a}\in \{ 0,1\}^{\mathcal{D}\times \mathcal{Q}^1}$. We use $X^{1a}_{dq}=1$ if and only if detection $d$ is associated with  $q$.  \alex{too many superscripts; can we avoid this?}

We associate each $q\in \mathcal{Q}^1$ with corresponding vectors $x^q,y^q,z^q$ as follows. 
$x^q_d=X^{1a}_{dq}$,$ y^q_{d_1d_2}=x^q_{d_1}x^q_{d_2}$,$z^q_d=X^{1a}_{dq}$.  
%\begin{align}
%\Theta_q=u(\theta,x) + p_1(\phi,y) + p_2(\phi,z,y) \quad  \forall q \in \mathcal{Q}^1
%\end{align}
Given $x^q,y^q,z^q$ we express the cost associated with $q\in \mathcal{Q}^1$ as follows.  

\begin{align}
\Theta_q=\sum_{d\in \mathcal{D}}\theta_dx^q_d +\sum_{\substack{d_1\in \mathcal{D}\\d_2\in \mathcal{D}}}\phi_{d_1d_2}y^q_{d_1d_2}(R_{d_1d_2}+z^1_{d_1}z^1_{d_2})\\
=\sum_{d\in \mathcal{D}}\theta_dx^q_d +\sum_{d_1,d_2 \in \mathcal{D}}x^q_{d_1}x^q_{d_2}\phi_{d_1d_2}
\end{align}

%For each part $r \in \mathcal{R}$ we define the set of all non-empty subsets of detections and selection of a unique single member of that set as $\mathcal{Q}^r$.  The union of $\mathcal{Q}^r$ for a ll r is denoted $\mathcal{Q}^0$ This unique member is denoted  global while the rest are local. 
We use $\mathcal{Q}^0$ to describe the set of  subsets of detections  where each subset  is assocaited with a single part  and where a single detection is labeled as global.  
We describe  $\mathcal{Q}^0$  using $X^{0a},X^{0b} \in \{0,1\}^{|\mathcal{D}| \times |\mathcal{Q}^r|}$. Here $X^{0a}_{dq}=1$ if and only if detection $d$ is assocaited with $q$ as a local detection.  Simlarly $X^{0b}_{dq}=1$ if and only if detection $d$ is assocaited with $q$ as a global detection.  

We assocaiate each $q\in \mathcal{Q}^0$ with corresponding vectors $x^q,y^q,z^q$ as follows. 
$x^q_d=X^{0a}_{dq}+X^{0b}_{dq}$,$ y^q_{d_1d_2}=x^q_{d_1}x^q_{d_2}$,$z^q_d=X^{0b}_{dq}$.  Costs of poses here are defined as in Eq\ref{costpose} minus the unary term on the global detection.
\begin{align}
\Theta_q=\sum_{d \in \mathcal{D}}\theta_d(x^q_d-z^q_d)+\sum_{d_1,d_2 \in \mathcal{D}}x^q_{d_1}x^q_{d_2}\phi_{d_1d_2}
\end{align}

We associate the members of $\mathcal{Q}^0,\mathcal{Q}^1$ with a vectors $\gamma^0 \in \{0,1\}^{|\mathcal{Q}^0|}$ and $\gamma^1 \in \{0,1\}^{|\mathcal{Q}^1|}$.  
We define a selection of local poses and global poses using $\gamma^0 \in \{0,1\}^{\mathcal{Q}^0},\gamma^1\in \{0,1\}^{\mathcal{Q}^1}$ respectively.  %We associate cost vectors $\Theta^0\in \mathbb{R}^{|\mathcal{Q}^1|} ,\Theta^1\in \mathbb{R}^{|\mathcal{Q}^1|}$ which are computed as in Eq \ref{costpose}.  %
Using this notation we write Eq \ref{eq:MainProg} using an equivelent form. We seek to find the lowest cost selection of poses hence we have an objective of  $\min_{\substack{\gamma^0 \in \{0,1\}^{|\mathcal{Q}^0|} \\ \gamma^1 \in \{0,1\}^{|\mathcal{Q}^1|}}}\Theta^{0t}\gamma^0+\Theta^{1t}\gamma^1 \\$

However we operate under the following hard constraints. 

1.  $X^{1a}\gamma^1+X^{0a}\gamma^0\leq 1$ no detection can be included as a global detection in a global pose or local detection in a local pose more than once

2.  $X^{0a}\gamma^0+X^{0b}\gamma^0\leq 1$ no detectection can be a global or local detection in more than one  local pose.  

3.  $-X^{1a}\gamma^1+X^{0b}\gamma^0\leq 0 $:  Every local detection must associated with a global detection of the same part. 

We write the objective and the above constraints below as an integer program

\begin{align}
\min_{\substack{\gamma^0 \in \{0,1\}^{|\mathcal{Q}^0|} \\ \gamma^1 \in \{0,1\}^{|\mathcal{Q}^1|}}}\Theta^{0t}\gamma^0+\Theta^{1t}\gamma^1 \\
\nonumber X^{1a}\gamma^1+X^{0a}\gamma^0\leq 1\\
\nonumber X^{0a}\gamma^0+X^{0b}\gamma^0\leq 1\\
\nonumber -X^{1a}\gamma^1+X^{0b}\gamma^0\leq 0
\end{align}

\section{Primal and Dual}

We now relax $\gamma$ to lie  in the positive orthant and observe its dual. 

\begin{align}
\min_{\substack{\gamma^0\geq 0 \\ \gamma^1 \geq 0}}\Theta^{0t}\gamma^0+\Theta^{1t}\gamma^1 \\
\nonumber X^{1a}\gamma^1+X^{0a}\gamma^0\leq 1\\
\nonumber X^{0a}\gamma^0+X^{0b}\gamma^0\leq 1\\
\nonumber -X^{1a}\gamma^1+X^{0b}\gamma^0\leq 0
\end{align}

Taking the dual of the relaxation introduces Lagrange multiplier sets  $\lambda^1,\lambda^2,\lambda^3 \in \mathbb{R}_{0+}^{|\mathcal{D}|}$

\begin{align}
\label{dualFormPose}
\max_{\substack{\lambda^1\geq 0\\ \lambda^2\geq 0 \\ \lambda^3\geq 0}} 1^t\lambda^1+1^t\lambda^2+1^t\lambda^3 \\
\nonumber \Theta^1+X^{1at}(\lambda^1-\lambda^3) \geq 0\\
\nonumber \Theta^0+X^{0at}\lambda^1+(X^{0at}+X^{0bt})\lambda^2+(X^{0bt})\lambda^3 \geq 0
\end{align}





==> columnLP.tex <==
\subsection{Reformulation of the Program}
\label{reform}
The LP relaxation of the ILP given in \ref{eq:MainProg} is very loose and does not provide solutions that can be rounded to good solutions. Instead we propose to solve Eq \ref{eq:MainProg} via an alternative technique known as delayed column generation\cite{barnprice}.  
%
Our integer program treats global and local interactions separately.  It constructs poses using a set of global and local poses that describe the global and local interactions respectively.  

Here a global pose describes all global key-points in a shared pose.  A local pose describes a set of key-points associated with a common part of which exactly one key-point is labeled as global. 

Our integer program should be understood as expressing a combinatorial number of poses from a set of global and local poses. This set is of exponential size and is referenced on demand using the Lagrangian dual. The creation of this set is discussed in broad terms in Section \ref{colgendef} and specific terms in Section \ref{violposes} and converted to an algorithm in Section \ref{colgenalg}.
%
%\subsection{Column Generation Approach}
%\label{colgendef}
%
%Column generation is a  key tool for solving  large scale  integer programs and is popular in the field of operations research~\cite{cuttingstock,barnprice}.  It is often associated with tight LP relaxations; fast inference and provable guarantees such as in correlation clustering \cite{PlanarCC} and cutting stock \cite{cuttingstock}.
%
%In general, column generation consists of writing an integer program over an exponential number of variables and a finite number of constraints.  Next the dual is taken which results in an finite number of variables and a exponential number of constraints.  \cite{lubbecke2010column} notes that every linear program with a finite number of variables can be solved in polynomial time via the ellipsoid algorithm if the most violated constraint can be identified in polynomial time.  In practice the ellipsoid algorithm is too slow and interior point or simplex methods are often used.  In this context the LP relaxation is solved followed by identifying additional violated constraints  in the dual.  Iterating this procedure until convergence yields a solution.  

%Often many violated constraints are added at once including the most violated.  Generating many constraints at once is often accomplished without extra computation as in ~\cite{HPlanarCC,yarkoNips2016} and in other cases can be done via parallel computation.  Each of these constraints corresponds to a primal variable.  Identifying violated constraints often consists of exactly solvable integer programs. At any time during or after termination a primal feasible LP relaxed solution to the original problem is produced by  relying only on the primal variables generated thus far. 

==> extTripOver.tex <==

\section{Extending Bounds to Triples }
\label{tripboundlocMe}
In this section we apply the techniques in Section \ref{bounPoseBase} to produce bounds on $\lambda^4$ and $\lambda^5$.  We write the corresponding LP below.   We use $\Omega^4 \in \mathbb{R}_+^{|\mathcal{C}^{\mathcal{G}}|}$,$\Omega^5\in \mathbb{R}_+^{|\mathcal{C}^{\mathcal{L}}|}$ to correspond to breaking the constraints corresponding to dual variables $\lambda^4$,$\lambda^5$.  The corresponding slack varaibles are denoted $\omega^4 \in \mathbb{R}_+^{|\mathcal{C}^{\mathcal{G}}|}$ and $\omega^5\in \mathbb{R}_+^{|\mathcal{C}^{\mathcal{L}}|}$

\begin{align}
\label{primalVerTripBOund2}
\mbox{Eq }\ref{primalTriRelax}=
\min_{\substack{\gamma \geq 0 \\ \psi \geq 0\\ \omega \geq 0}}\Gamma^t \gamma +\Psi^t \psi+ \Omega^{1t}\omega^1+\Omega^{4t}\omega^4+\Omega^{5t}\omega^5 \\
\nonumber G^t\gamma+L^t\psi -\omega^1\leq 1 \\
\nonumber M^t \psi+L^t\psi \leq 1\\
\nonumber -G^t\gamma +M^t\psi\leq 0\\
\nonumber C^{\mathcal{G}}\gamma-\omega^4 \leq 1\\
\nonumber C^{\mathcal{L}}\psi-\omega^5 \leq 1\\
=
\max_{\lambda \geq 0 } -1^t\lambda^1-1^t\lambda^2-1^t\lambda^3-1^t\lambda^4-1^t\lambda^5 \\
\nonumber \Gamma+G^t(\lambda^1-\lambda^3)+C^{\mathcal{G}t}\lambda^4 \geq 0 \\
\nonumber \Psi+L^t\lambda^1+(M^t+L^t)\lambda^2+M^t\lambda^3 +C^{\mathcal{L}t}\lambda^5 \geq 0 \\
\nonumber \Omega^1\geq \lambda^1\\
\nonumber \Omega^4\geq \lambda^4\\
\nonumber \Omega^5\geq \lambda^5
\end{align}



==> lp_one_legacy.tex <==

\subsection{ILP One:  Set Packing Formulation}
In this section we write the program given in \equref{eq:MainProg} as a set packing problem.  In this formulation, poses of entire people which we refer to as `complete poses' are variables.  Costs of `complete poses' are derived from the cost terms in \equref{eq:MainProg}.  The objective of set packing is to select a set of low cost poses such that none of the selected poses share a common detection.  

We define the exponential sized set of all complete poses using  $\mathcal{Q}$. % and index it with $q$.  
We describe these poses using matrices $X^{0},X^1 \in \{ 0,1\}^{|\mathcal{D}|\times|\mathcal{Q}|}$.  Hereby $X^0_{dq}=1$ indicates that detection $d$ is associated with  complete pose  $q$ and is a local detection.   We use $X^1_{dq}=1$ to indicate that  $q$ includes detection $d$ as a global detection.  

The $x$,$y$, and $z$ vectors corresponding to a complete pose $q\in\mathcal{Q}$ are written as $x^q,y^q,z^q$.  Given solutions for $X^0$ and $X^1$, we infer the corresponding  solution for the original variables via $x^q_d=X^0_{dq}+X^1_{dq}$, $y_{d_1d_2}=(X^0_{d_1q}+X^1_{d_1q})(X^0_{d_2q}+X^1_{d_2q})$, and $z^q_d=X^1_{dq}$.  \alex{the reader likely wants to know how we obtain those solutions? we need to provide intuition for it.}

We describe a selection of complete poses as $\gamma \in \{ 0,1 \}^{|\mathcal{Q}|}$.  A selection of poses must obey the constraint that no two selected poses share a common detection.  This is enforced via  $(X^0+X^1)\gamma \leq 1$.  

%
%
We  associate the set of complete poses  with a vector  of costs $\Theta \in \mathbb{R}^{\mathcal{Q}}$ which is indexed by $q$.   Here $\Theta_q$ is the cost associated with complete pose $q$.  Thus $\Theta_q=$ \alex{something missing}


We define  $\Theta_q$ using the notation in \equref{eq:MainProg} as follows.  

\alex{I don't understand the following equation; need more intuition}
\begin{align}
\label{costpose}
\Theta_q=\sum_{d\in \mathcal{D}}\theta_dx^q_d +\sum_{\substack{d_1\in \mathcal{D}\\d_2\in \mathcal{D}}}\phi_{d_1d_2}y^q_{d_1d_2}(R_{d_1d_2}+z^1_{d_1}z^1_{d_2})\\
%
\nonumber =\sum_{d\in \mathcal{D}}\theta_dx^q_d +\sum_{\substack{d_1\in \mathcal{D}\\d_2\in \mathcal{D}}}\phi_{d_1d_2}(R_{d_1d_2}+z^1_{d_1}z^1_{d_2})
\end{align}


We now frame  the program given in \equref{eq:MainProg} as a set packing task via:
\begin{align}
\label{packingIlp}
\mbox{Eq } \ref{eq:MainProg}=\min_{\substack{\gamma \in \{ 0,1\}^{|\mathcal{Q}|} \\ (X^0+X^1)\gamma \leq 1}}\Theta^t\gamma 
\end{align}



==> old_intro.tex <==
\section{Introduction}
%In this paper we study the problems of multiple pose segmentation given natural images and crowded cells in bioimages.
We consMultiple pose segmentation  ~\cite{deepcut1,deepcut2} is the problem of jointly inferring the pose of multiple people given an image.  It is a challenging problem with applications in areas as diverse as entertainment and  security.

Classical methods for determining the pose of people are based on deformable part models\cite{deva1,deva2,deva3}.  These model human pose according to a tree structured Markov Random Field with efficient inference based on distance transforms. %Therefore, we formulate multiple-pose segmentation from the perspective of grouping disjoint sets of detections of parts called key-points  into poses whose underlying structure is modeled using traditional tree shaped deformable part based models. 

Our work on pose segmentation is based on the work of \cite{deepcut1,deepcut2} which frames multiple pose segmentation as a massive integer linear program.  They tackle it with exact inference using the CPLEX integer linear program solver.  Our work is distinct from \cite{deepcut1,deepcut2} primarily via the approach that we apply to inference.  We rely on column generation \cite{cuttingstock,barnprice} approaches methods tailored specifically to multiple pose segmentation. To facilitate efficient inference some parts of the model of  \cite{deepcut1,deepcut2} are altered.  
%Our work is closely related to \cite{HPlanarCC}.  Here the authors  attack inference in image partitioning using delayed column generation\cite{cuttingstock,barnprice}, where columns correspond to a basis set of 2-colorable partitions.  The authors found that column generation on its own was insufficient as the set of columns grew too slowly.  They were able to establish bounds on the Lagrange multipliers in the dual which in turn could be interpreted as a massive number of additional columns that exist implicitly and thus do not slow down inference.  We apply this same trick to gain the effect of having more columns than we actually can produce.  
Our work is most closely related to \cite{yarkoNips2016}.  In this paper the authors frame multiple object tracking from the perspective of maximum weight set packing.  Track costs are derived from a non first order Markov chain.  Tracks are generated in large quantities using dynamic programming. The corresponding LP relaxation is generally tight but the authors further tighten it using third order odd set inequalities \cite{heismann2014generalization}.%  These correspond to the higher order constraints of \cite{sontag}.  
	
Like \cite{deepcut1,deepcut2,ZhangSchwingICCV2015} we rely on deep convolutional neural networks (CNN) trained via gradient descent learning \cite{hinton} to produce costs for our optimization problems.  
CNN are mathematical approximations to large groups of neurons that are trained on large quantities of data and have been demonstrated to provide state of the art performance on numerous tasks including in computer vision \cite{krizhevsky2012imagenet,wu2015deep}, speech recognition \cite{hinton2012deep}, and exotic particle search \cite{baldi2014searching}.
%
\subsection{Cell Instance Segmentation}
%
Recent advances in microscope techniques, automation, long-term high-throughput imaging, etc, result in a vast amount of data in biological experiments, making traditionally manual analysis on these images infeasible. Accurately segmenting a large number of objects of similar type in crowded images is challenging, e.g. when cells of interest touch or overlap. To enable generality, less human interaction, unsupervised image segmentation algorithms often are popular. Typically they start with an over-segmentation into superpixels, which are then clustered into ``perceptually meaningful" regions~\cite{Zhang14b}. 

Our work on cell instance segmentation is  related to \cite{ZhangSchwingICCV2015}. In this work the authors use depth to transform instance segmentation into a labeling problem and thus break the difficult symmetries found when studying the problem.  They frame optimization as an integer linear program and attack it using the greedy methods of network flows \cite{boykov2001fast} notably Quadratic Pseudo-Boolean Optimization \cite{rother2007optimizing,boros2002pseudo}.  This requires specific knowledge about the number of labels present in the image.  Our work in contrast uses an integer linear programming framework that does not require knowing the number of labels present in the image.  Inference is conducted using an LP relaxation that is tightened using cutting plane methods as in \cite{yarkoNips2016}.
%

==> pose_bound_basic.tex <==
\section{Bounding the Lagrange Multipliers}
\label{bounPoseBase}
%
Inspired by the work of \cite{PlanarCC,HPlanarCC}, we observe that before convergence of  column generation the optimal solution may not lie in the span of the set of columns produced thus far.   It is useful to allow some values of $G\gamma+L\psi$  to exceed one.  We introduce a slack vectors $\omega^1$ that tracks the presence of any ``over-included" key-points  and prevents them from contributing to the objective when that contribution is negative. 
%
The result of this is bounds on the dual variables $\lambda^1$ that can speed convergence of optimization. The study of similar bounds on $\lambda^4,\lambda^5$ is addressed in Section \ref{tripboundlocMe}.   

%In this section we consider the problem of providing bounds to the dual variables  $\lambda^1$.  
We organize this section as follows. In Section \ref{motiv} we motivate the use of bounds on $\lambda^1$ in terms of the primal problem. This results in a relaxed set of constraints relative to Eq \ref{primalTriRelax}.  In Section \ref{drop1} we propose an algorithm that projects a solution on the relaxed constraint set  onto the non-relaxed constraint set.  These updates decrease the objective.  %In Section \ref{observeOmega} we observe the change in the objective as a result of the updates to the primal solution.  
%
%The algorithm however is not implemented in our code it is simply used to demonstrate that the bounds on the Lagrange multipliers do not alter the primal solution at convergence of column generation or column/row generation.  We then upper bound this change.  This upper bound is then used to%Given the upper bound we set $\Omega$ so as to ensure that the value of this upper bound is negative.  
 %
\subsection{Motivation in the Primal for Bounds}
\label{motiv}
Consider that we have two very low cost global poses and that they overlap at a single key-point $d_1$ corresponding to a non-global part.  Furthermore assume that the strength of the pairwise connections between $d_1$ and its neighbors are very weak.  It seems wasteful to not use both global poses; however the hard constraint that $G\gamma+L\psi\leq 1$ prevents the use of both in the solution.  To circumvent this issue we allow ourselves to violate the constraint at a cost  $\Omega^{1} \in \mathbb{R}^{\mathcal{D}}_{+}$.  %Here $$ the cost for violating the constraint. 
We define $\Omega^1$ such that its introduction does not alter the objective given the full set of columns.  We describe primal and dual optimization augmented with the primal slack vector $\omega^1$ as follows. 
%
%However consider that we associate a cost to removing $d_1$ from an arbitrary pose.  This cost is defined such that 
% we apply the following.  
%IThe LP resultant LP is as follows.  
\begin{align}
\label{primalVerTripBOund}
\mbox{Eq }\ref{primalTriRelax}=
\min_{\substack{\gamma \geq 0 \\ \psi \geq 0\\ \omega \geq 0}}\Gamma^t \gamma +\Psi^t \psi+ \Omega^{1t}\omega^1 \\
\nonumber G^t\gamma+L^t\psi -\omega^1\leq 1 \\
\nonumber M^t \psi+L^t\psi \leq 1\\
\nonumber -G^t\gamma +M^t\psi\leq 0\\
\nonumber C^{\mathcal{G}}\gamma \leq 1\\
\nonumber C^{\mathcal{L}}\psi \leq 1\\
=
\max_{\lambda \geq 0 } -1^t\lambda^1-1^t\lambda^2-1^t\lambda^3-1^t\lambda^4-1^t\lambda^5 \\
\nonumber \Gamma+G^t(\lambda^1-\lambda^3)+C^{\mathcal{G}t}\lambda^4 \geq 0 \\
\nonumber \Psi+L^t\lambda^1+(M^t+L^t)\lambda^2+M^t\lambda^3 +C^{\mathcal{L}t}\lambda^5 \geq 0 \\
\nonumber \Omega^1\geq \lambda^1
\end{align}
%
Observe that the introduction of $\Omega^1$ adds an upper bound $\lambda^1$ in the dual.  Clearly if we set $\Omega^1$ to be infinite then $\omega^1$ will be zero.  Also observe that by definition $\omega^1$ is zero valued at termination.  However prior to convergence of column generation the primal solution of the relaxed problem in Eq \ref{primalVerTripBOund} may have lower cost than the unrelaxed problem in Eq \ref{primalTriRelax} if $\Omega^1$ is non-infinite. 

We consider the construction of $\Omega^1$ satisfying the constraint that Eq \ref{primalTriRelax}=Eq \ref{primalVerTripBOund}.  Our $\Omega$ term is infinite for key-points corresponding to global parts but non-infinite for key-points corresponding to non-global parts.  %We consider only $d$ corresponding to non-global parts.  We now introduce a proceadure that 

==> pose_bound_mult.tex <==

\section{UNDER CONSTRUCTION Bounding the Lagrange multipliers}

In this section we consdier the problem of providing bounds to the dual varaibles  $\lambda^1$ and $\lambda^4$.  We organize this section as follows. In Section \ref{motiv} we motivate the use of bounds on the dual variables  in terms of the primal problem.  In Section \ref{propBound} we assert a bound on $\lambda^1$ and $\lambda^4$.  In Section \ref{drop1} we propose an algorithm that projects a solution onto the relaxed constraint set  onto the non-relaxed constraint set.  This is done in two steps first for $\lambda^1$ in Section \ref{lam1drop} adn for $\lambda^4$ in Section \ref{lam4drop}
 
\subsection{Motivation in the primal}
\label{motiv}
Consider that we have two global poses and that they overlap at a single key-point $d_1$ corresponding to a non-global part.  Furthermore assume that the strength of the pairwise connections between $d_1$ and its neighbors are very weak.  It seems wasteful to not be able to use both global poses.  However the hard constraint that $G\gamma+L\psi\leq 1$ prevents the use of both in the solution.

% we apply the following.  
Inspired by the work of \cite{PlanarCC,HPlanarCC}, we observe that before convergence of  column generation the optimal solution may not lie in the span of the set of columns.   It is useful to allow some values of $G\gamma+L\psi$  and $C^{\mathcal{G}}\gamma$ to exceed one.  We introduce a slack vectors $\beta^1$ and $\beta^4$ that track the presence of any ``over-included" key-points  and prevents them from contributing when that contribution is negative. 

The LP resultant LP is as follows.  
\begin{align}
\min_{\substack{\gamma \geq 0 \\ \psi \geq 0\\ \omega \geq 0}}\Gamma^t \gamma +\Psi^t \psi+ \Omega^{1t}\omega^1+ \Omega^{4t}\omega^4+\Omega^{5t}\omega^5 \\
\nonumber G^t\gamma+L^t\psi -\omega^1\leq 1 \\
\nonumber M^t \psi+L^t\psi \leq 1\\
\nonumber -G^t\gamma +M^t\psi\leq 0\\
\nonumber C^{\mathcal{G}}\gamma -\omega^4 \leq 1\\
\nonumber C^{\mathcal{L}}\psi \omega^5 \leq 1
\end{align}
In the dual we observe the following.  The introduction of $\omega$ induces bounds on $\lambda$.  We write these below.  
\begin{align}
\max_{\lambda \geq 0 } -1^t\lambda^1-1^t\lambda^2-1^t\lambda^3-1^t\lambda^4-1^t\lambda^5 \\
\nonumber \Gamma+G^t(\lambda^1-\lambda^3)+C^{\mathcal{G}t}\lambda^4 \geq 0 \\
\nonumber  \Psi+L^t\lambda^1+(M^t+L^t)\lambda^2+M^t\lambda^3 +C^{\mathcal{L}t}\lambda^5 \geq 0 \\
\nonumber \Omega^1\leq \lambda^1\\
\nonumber \Omega^4\leq \lambda^4\\
\nonumber \Omega^5\leq \lambda^5
\end{align}

Clearly if we set $\Omega^1,\Omega^4$ to be infinite then $\omega^1,\omega^4$ will be zero.  However we establish a value such that at any point in optimization we can prove that a lower cost solution can be achieved by adding more columns.   



==> pose_bound_sim_old.tex <==
\subsection{Projecting $\omega^1$}
\label{drop1}
%
We now consider the construction of a bound on $\Omega^1$.  This bound is defined to be infinite for all $d$ associated with a global part and non infinite otherwise.    

We now consider a procedure that iterates through $d$ such that $R_d\notin \hat{\mathcal{R}}$ and $\omega_d>0$.  %After each iteration we retain a feasible solution to Eq \ref{primalVerTripBOund}.  %When $\omega_d>0$ our procedure 
After each iteration  our procedure updates terms in $\gamma,\psi$ so as to achieve the following 3 goals  for a given $d \in \mathcal{D}$.
\begin{itemize}
\item Decrease the objective
\item Remain Feasible
\item Decrease or leave constant all $\omega$ terms
\item  set $\omega^1_{d}$ to zero
\end{itemize} 
%

For any selection of $d_* \in \mathcal{D}$ we  consider a mapping of poses $q$ to a corresponding $\bar{q}$.  Our mapping is defined only for global poses where $G_{d_*q}=1$ and local poses where $L_{d_*q}=1$. For a given global pose $q$ such that $G_{d_*q}=1$ the corresponding pose $\bar{q}$ is identical to q except that $G_{d_*\bar{q}}=0$.  For a given local pose $q$ such that $L_{d_*q}=1$ the corresponding pose $\bar{q}$ is identical to q except that $L_{d_*\bar{q}}=0$.  
%
%Similarly for a local pose $q$ where $d_*$ is a local key-point $\bar{q}$ is the pose $d_*$ removed if $d_*$ is present in $q$.  In the case where $d_*$ is the global part in $q \in \mathcal{L}$ then $\bar{q}$ does not exist. % is the ``empty pose". The empty pose has no key-points associated with it and has zero cost.  %describe the set of poses both global and local in terms of removing element $d$ if present.  For any given $q$ we define Let $\bar{q}_{d_*}$ be defined as follows
%
We define this mapping below.  
%
\begin{align}
G_{d\bar{q}}=G_{dq}[d\neq d_*]\quad \forall d \in \mathcal{D}, q\in \mathcal{G}\quad  G_{d_*q}=1\\
%\nonumber M_{d\bar{q}}=M_{dq}[d \neq d_*] \quad \forall d \in \mathcal{D}, q\in \mathcal{L} \quad \\
\nonumber M_{d\bar{q}}=M_{dq} \quad \forall d \in \mathcal{D}, q\in \mathcal{L}\quad L_{d_*q}=1\\
\nonumber L_{d\bar{q}}=L_{dq}[d\neq d_*]\quad \forall d \in \mathcal{D}, q\in \mathcal{L}\quad L_{d_*q}=1%(1-\sum_{d_1 \in \mathcal{D}}M_{d_1q} d_1)
\end{align}
%
%We now consider an update to $\psi,\gamma$ that enforces the constraint corresponding to key-point $d_*$ in the constraint sets $G\gamma+L\psi \leq1$ and $-G\gamma+M\psi \leq 1$.  We write the constraint that is enforced by our update below.    
%\begin{align}
%G_{d_*,:}\gamma+L_{d_*,:}\psi \leq 1\\
%\nonumber -G_{d_*,:}\gamma+M_{d_*,:}\psi \leq 0
%\end{align}
%
We now consider our update to $\psi,\gamma$.   %We define the change to $\gamma_q$ or $\psi_q$ terms using $\delta$ indexed by $q$ written below
After the updates are applied we set $\omega^1_{d_*}=0$. The updates that achieve this are written below.  % We now discuss the change in the value of the objective achieved via these updates in terms of $\gamma,\psi,\omega$
%
\begin{align}
\label{updateEquDelta}
\gamma^{\mbox{NEW}}_q= \gamma_q-\gamma_q\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}} \quad  \forall q \in \mathcal{G}, G_{d_*q}=1\\
\nonumber \psi^{\mbox{NEW}}_q= \psi_q-\psi_q\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}} \quad \forall q \in  \mathcal{L};\; (M_{d_*q}+L_{d_*q}=1) \\
\nonumber  \gamma^{\mbox{NEW}}_{\bar{q}}= \gamma_{\bar{q}}+\gamma_q\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}\quad \forall q \in \mathcal{G};G_{d_*q}=1\\
\nonumber \psi^{\mbox{NEW}}_{\bar{q}}=\psi_{\bar{q}}+ \psi_q\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}[\Psi_{\bar{q}}<0] \quad \forall q \in \mathcal{L};\quad L_{d_*q}=1
%\omega^{\mbox{NEW}}_{d_*}=0
\end{align}
%
%
These updates describe why we only consider $d_* \in \mathcal{R}_d$.  Recall that  a pose must include a key-point corresponding to a global part.  If the updates in Eq \ref{updateEquDelta} were applied on $d_*$ where $d_*\in \hat{ \mathcal{R}}$ then poses that have a no key-point corresponding to a global part could be introduced into the solution.  Hence we set $\Omega^1_{d}=\infty$ for all $d$ such that $R_d\in \mathcal{R}$.  That way the corresponding terms in $\omega$ are guaranteed to be zero valued.  

After the updates in Eq \ref{updateEquDelta} are applied for any given $d_* \in \mathcal{D}$ it may be the case that $\omega$ terms can be decreased leaving $\gamma$ and $\psi$ fixed.  These updates can not increase the objective and are written below.  %loosen some constraints defining  $\omega^1,\omega^4,\omega^5$ to become loose for active terms.  Thus we decrease the corresponding $\omega$ terms as follows.  Any resulting alteration to $\omega^1$ decreases the objective.  
%
\begin{align}
\label{updateOmegaEZ}
\omega^1_d\leftarrow \max[0,G_{d,:}\gamma^{\mbox{NEW}}+L_{d,:}\psi^{\mbox{NEW}}-1] \quad \forall d \in \mathcal{D}\\
\nonumber \omega^4_c=\max[0,C^{\mathcal{G}}_c\gamma^{\mbox{NEW}}-1] \quad \forall c \in \mathcal{C}^{\mathcal{G}}\\
\nonumber \omega^5_c=\max[0,C^{\mathcal{L}}_c\psi^{\mbox{NEW}}-1]\quad  \forall c \in \mathcal{C}^{\mathcal{L}}
\end{align}
%
%
%
\subsubsection{Establishing the value of  $\Omega^1_{d_*}$}
\label{observeOmega}
%
We denote the  change in the objective achieved by the updates in Eq \ref{updateEquDelta}  as $\Delta$ which we define below. %
\begin{align}
\label{DeltaEq}
\Delta=-\omega^1_{d_*}\Omega^1_{d_*}+\sum_{q\in \mathcal{G}}\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}\gamma_qG_{d_*q}(\Gamma_{\bar{q}}-\Gamma_q)+\sum_{q\in \mathcal{L}}\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}\psi_q(L_{d_*q}+M_{d_*q})(\Psi_{\bar{q}}L_{d*q}[\Psi_{\bar{q}}<0]-\Psi_q)\\
%
\nonumber =\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}\gamma_q(\Gamma_{\bar{q}}-\Gamma_q)+\sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q(\Psi_{\bar{q}}[\Psi_{\bar{q}}<0]-\Psi_q)+\sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\psi_q(0-\Psi_q))
\end{align}
%
From Eq \ref{DeltaEq} we know that in order for $\Delta$ to be negative the following must hold for any solution $\gamma,\psi$.
%
\begin{align}
\label{mustsatis}
(1+\omega^1_{d_*})\Omega^1_{d_*}>\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}\gamma_q(\Gamma_{\bar{q}}-\Gamma_q)+\sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q(\Psi_{\bar{q}}[\Psi_{\bar{q}}<0]-\Psi_q)+\sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\psi_q(0-\Psi_q))
\end{align}
%
Thus Eq \ref{mustsatis} defines the conditions for a suitable  $\Omega^1_{d_*}$. To identify a suitable value $\Omega^1_{d_*}$ we produce an upper bound on Eq \ref{DeltaEq} and set $\Omega^1_{d_*}$ accordingly.  The resultant value on  $\Omega^1_{d_*}$ term is strictly greater than the term needed to satisfy Eq \ref{mustsatis}.  

We now proceed to upper bound Eq \ref{DeltaEq}.  We achieve this using terms $\alpha_1,\alpha_2,\alpha_3 \in \mathbb{R}_{0+}$ defined as follows.
%
\begin{align}
\alpha_1:\quad \max[0,\max_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}(\Gamma_{\bar{q}}-\Gamma_q)] =\max[0,\max_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}-\theta_{d_*}+\sum_{d_1\neq d}\theta_{d_*d_1}G_{d_1q}] \\
\nonumber \leq \max[0,-\theta_{d_*}-\sum_{\substack{r \in \mathcal{R}\\ r \neq R_{d_*}}}\min[0,  \min_{\substack{d_1 \in \mathcal{D}\\R_{d_1}=r}} \phi_{d_*d_1}]]=\alpha_1\\
%\min[0,\min_{\substack{d_1 \in \mathcal{D}\\[R_d=r]}}\phi_{d_*d_1}]
%
\nonumber \alpha_2:\quad \max[0,\max_{\substack{q\in \mathcal{L}\\L_{d_*q}=1}}(\Psi_{\bar{q}}[\Psi_{\bar{q}}<0]-\Psi_q)] =\alpha_2\\
% \leq \max[0,\max_{\substack{q\in \mathcal{L}\\L_{d_*q}=1}}(-\Psi_q)] =\alpha_2\\
\nonumber \alpha_3: \quad \max[0,\max_{\substack{q\in \mathcal{L}\\M_{d_*q}=1}}((0-\Psi_q))]=\alpha_3
\end{align}
%
Observe that $\alpha_1$ can be computed by checking each pairwise term including key-point $d_*$.  We compute $\alpha_2,\alpha_3$ via exhaustive search.  The computation of  $\alpha_2,\alpha_3$ is tractable because we did not  have more than fifteen key-points per part in any problems in our data set and hence we only had $2^{15}$ possible $q$ to consider.  %Since for each part we did not have more than fifteen key-points for any given part  in general for our problem instances  and generally less than ten we found this search to not be problematic.  

We write our first upper bound on  Eq \ref{DeltaEq} as follows.  
\begin{align}
\label{deltaStep2}
\mbox{Eq } \ref{DeltaEq} \leq  \frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+\alpha_1\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}\gamma_q+\alpha_2\sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q+\alpha_3\sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\gamma_q)
\end{align}
%
Given that $-G_{d,:}\gamma+M_{d,:}\psi \leq 0$ and that  $\alpha_3\geq 0$ we conclude the following. % to produce the following upper bound on . 
\begin{align}
\label{boundTrick}
\alpha_3\sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\gamma_q\leq \alpha_3\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}\gamma_q
\end{align}
%
%can upper bound  \sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\gamma_q$ by  Eq \ref{deltaStep2} by as follows 
We use Eq \ref{boundTrick} to upper bound Eq \ref{deltaStep2} below. 
\begin{align}
\label{deltaStep3}
\mbox{Eq }\ref{deltaStep2} \leq \frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+(\alpha_1+\alpha_3)\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}  \gamma_q+\alpha_2 \sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q)%+\sum_{\substack{q\in \mathcal{L}\\ M_{d_*q}=1}}\alpha_3)
\end{align}
%
We now upper bound Eq \ref{deltaStep3} by  replacing $\alpha_1+\alpha_3$ and $\alpha_2$ with $\max[\alpha_1+\alpha_3,\alpha_2]$.  
%
\begin{align}
\label{deltaStep4}
\mbox{Eq }\ref{deltaStep3} \leq %\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+\max[\alpha_1+\alpha_3,\alpha_2]\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}}  \gamma_q+\max[\alpha_1+\alpha_3,\alpha_2] \sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q \\
 \frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+ \max[\alpha_1+\alpha_3,\alpha_2](\sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q+\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}} \gamma_q))
\end{align}
%
Recall that $G_{d_*,:}\gamma+L_{d_*,:}\psi \leq 1+\omega^1_{d_*}$ and that $\max[\alpha_1+\alpha_3,\alpha_2]$ is non-negative. We therefor establish the following.    %
\begin{align}
 \max[\alpha_1+\alpha_3,\alpha_2](\sum_{\substack{q\in \mathcal{L}\\ L_{d_*q}=1}}\psi_q+\sum_{\substack{q\in \mathcal{G}\\G_{d_*q}=1}} \gamma_q)) \leq  \max[\alpha_1+\alpha_3,\alpha_2] (1+\omega^1_{d_*})
\end{align}
%
We now upper bound Eq \ref{deltaStep4} by replacing $G_{d_*,:}\gamma+L_{d_*,:}\psi$ with $1+\omega^1_{d_*}$.%
%Thus we can upper bound Eq \ref{deltaStep4} as follows.
%
\begin{align}
\mbox{Eq }\ref{deltaStep4}=\frac{\omega^1_{d_*}}{1+\omega^1_{d_*}}(-(1+\omega^1_{d_*})\Omega^1_{d_*}+ \max[\alpha_1+\alpha_3,\alpha_2](1+\omega^1_{d_*}))\\
\nonumber =\omega^1_{d_*}(-\Omega^1_{d_*}+ \max[\alpha_1+\alpha_3,\alpha_2])
\end{align}
%
In order to ensure that $\Delta <0$ it is sufficient to ensure that $\Omega^1_{d_*}> \max[\alpha_1+\alpha_3,\alpha_2])$
%
%In order to establish $\Omega^1_{d_*}$ we need to study the values $\alpha_1,\alpha_2,\alpha_3$
%
Let $\epsilon$ be a tiny positive number.  We now define $\Omega^1_{d_*}$.  
\begin{align}
\Omega^1_d=\epsilon+\max[\alpha_1+\alpha_3,\alpha_2]
\end{align}
%
%\subsubsection{Optimality Guarantee}
%
%At termination any alteration to $\$
%This procedure may associate non-zero $\gamma$ terms with columns that are not available in the set of columns at a given stage of column generation.  However at termination of column generation the solution has value equal to optimization over all columns.  Hence at termination $\omega^1$ must be a zero vector. 

==> scratch_trip.tex <==

\subsection{on local triples }

For each $c\in \mathcal{C}^{\mathcal{L}}$; $c=[d_1,d_2,d_3]$.  Let $d_1$ be the maximizer term for $c$  in $\Omega$.
\begin{align}
M_{d\bar{q}}=M_{dq}(\max(1-[d~=d_2][d~=d_3],1-C^L_{cq}))\\
\nonumber L_{d\bar{q}}=L_{dq}(\max([d~=d_2][d~=d_3],1-C^L_{cq}))\sum_{d_a}M_{d_a\bar{q}}
\end{align}
%
\begin{align}
\delta_q\leftarrow -\psi_q(L_{d_*q}+M_{d_*q})\frac{\omega_{d_*}}{1+\omega_{d_*}} \quad \forall q \in  \mathcal{L} \\
\nonumber \delta_{\bar{q}}\leftarrow \psi_q(L_{d_*q}+M_{d_*q})\frac{\omega_{d_*}}{1+\omega_{d_*}}[\Psi_{\bar{q}}<0] \quad \forall q \in \mathcal{L} 
\end{align}
%
%
%
\begin{align}
\label{DeltaEqLOC}
\Delta=-\omega_{c}\Omega_{c}+\sum_{q\in \mathcal{L}}\frac{\omega_{c}}{1+\omega_{c}}\psi_qC^L_{cq}([\Psi_{\bar{q}}<0]-\Psi_q)\\
%
\nonumber =\frac{\omega_{d_*}}{1+\omega_{c}}(-(1+\omega_{d})\Omega_{c}+\sum_{q\in \mathcal{L}}\psi_qC^L_{cq}([\Psi_{\bar{q}}<0]-\Psi_q)
\end{align}

%By definition of the inequality $C\psi-\omega^4\leq 1$ and that $\omega^4$ is a positive vetor we know that  $\sum_{q\in \mathcal{L}}\frac{\omega_{c}}{1+\omega_{c}}\psi_q=1+\omega_c$

%We now seek to upper bound Eq \ref{DeltaEqLOC}.  We do this  as follows 
%Thus Eq \ref{DeltaEqLOC} can be rewritten as follows.  
%\begin{align}
%\label{DeltaEqLOC2}
% \mbox{Eq }\ref{DeltaEqLOC}=\omega_{c}(-\Omega_{c}+\sum_{q\in \mathcal{L}}\psi_qC^L_{cq}(\Psi_{\bar{q}}[\Psi_{\bar{q}}<0]-\Psi_q)) 
%\end{align}

We now upper bound Eq \ref{DeltaEqLOC} as follows
\begin{align}
\mbox{Eq }\ref{DeltaEqLOC}\leq \frac{\omega_{c}}{1+\omega_{c}}(-(1+\omega_{c})\Omega_{c}+\sum_{q\in \mathcal{L}}\psi_qC^L_{cq}(-\Psi_q)
\end{align}

We now upper bound $C^L_{cq}(-\Psi_q)$ using a term $\alpha$ defined as follows.  Note that 

\begin{align}
\alpha=\max_{q \in \mathcal{L}}C^L_{cq}(-\Psi_q)
\end{align}
Using $\alpha$ we can upper bound \mbox{Eq }\ref{DeltaEqLOC} as follows.  
\begin{align}
\label{DeltaEqLOC2}
\mbox{Eq }\ref{DeltaEqLOC}\leq \frac{\omega_{d_*}}{1+\omega_{c}}(-(1+\omega_{d})\Omega_{c}+\sum_{q\in \mathcal{L}}\psi_qC^L_{cq}\alpha
\end{align}


